Compact Lattice Gadget and Its Applications to Hash-and-Sign Signatures

This work aims to improve the practicality of gadget-based cryptosystems, with a focus on hash-and-sign signatures. To this end, we develop a compact gadget framework in which the used gadget is a square matrix instead of the short and fat one used in previous constructions. To work with this compact gadget, we devise a specialized gadget sampler, called semi-random sampler, to compute the approximate preimage. It first deterministically computes the error and then randomly samples the preimage. We show that for uniformly random targets, the preimage and error distributions are simulatable without knowing the trapdoor. This ensures the security of the signature applications. Compared to the Gaussian-distributed errors in previous algorithms, the deterministic errors have a smaller size, which lead to a substantial gain in security and enables a practically working instantiation. As the applications, we present two practically efficient gadget-based signature schemes based on NTRU and Ring-LWE respectively. The NTRU-based scheme offers comparable efficiency to Falcon and Mitaka and a simple implementation without the need of generating the NTRU trapdoor. The LWE-based scheme also achieves a desirable overall performance. It not only greatly outperforms the state-of-the-art LWE-based hash-and-sign signatures, but also has an even smaller size than the LWE-based Fiat-Shamir signature scheme Dilithium. These results fill the long-term gap in practical gadget-based signatures.

==> app_security.tex <==
%!TEX root = main.tex
\section{Proof of Theorem~\ref{thm:Robinsecurity}}\label{appendix:securityproof}
%\subsection{Proof of Theorem~\ref{thm:Robinsecurity}}
\begin{proof}
  Suppose, for contradiction, that there is an adversary $\mathcal A$ that breaks the strong EU-CMA security of \Robin{} with non-negligible probability $\varepsilon$.
  We construct a polynomial time algorithm $\mathcal S$ that solves $\mathsf{NTRUSIS}^{\|\cdot\|_\gamma}_{\cR,Q,\chi,2\beta}$ with probability close to $\varepsilon$. 
  Given a random NTRU public key $h$, $\mathcal S$ runs
  %Given matrix $\mathbf A$ in the Hermite normal form, which defines function $f_{\mathbf A}(\cdot):\mathbb Z^m\rightarrow\mathbb Z_q^n$,
  $\mathcal A$ and simulates the random oracle $\mathsf H$ and signing oracle as follows:

  \begin{itemize}
    \item for the query to $\mathsf H$ on $(\mathsf{salt,msg})$, 
    if $\mathsf H(\mathsf{salt,msg})$ is not queried, then 
    $\mathcal S$ samples $(\vecz=(z_0,z_1), e)\gets D_{\mathbb Z^{2n},s} \times U(\mathbb Z_p^n)$, 
    returns $u = z_0+z_1h+e\mod Q$ as the random oracle response and stores 
    $((\mathsf{salt,msg}),z_0,z_1,e,u)$. 
    Otherwise $\mathcal S$ looks up $((\mathsf{salt,msg}),z_0,z_1,e,u)$ and returns $u$ to $\mathcal A$.
    
%    $\mathcal S$ samples $\mathbf z=(z_0,z_1)\leftarrow D_{\mathbb Z^{2n},s}$ and $\mathbf e\leftarrow U(\mathbb Z_p^n)$, then returns $\mathbf{u=Az+e}\mod Q$ to $\mathcal A$. If $\mathsf H$ was previously queried on $(\mathsf{salt,msg})$, $\mathcal S$ looks up $((\mathsf{salt,msg}),\mathbf{z}_0,\mathbf z_1, \mathbf{e,u})$ and returns $\mathbf u$.
	\item for every signing query on $\mathsf{msg}$, $\mathcal S$ samples $\mathsf{salt}\overset{\$}{\leftarrow}\{0,1\}^{320}$, 
	$(\vecz=(z_0,z_1), e)\gets D_{\mathbb Z^{2n},s} \times U(\mathbb Z_p^n)$, then outputs $(\mathsf{salt},z_1)$ to $\mathcal A$ as the signature, and stores $((\mathsf{salt,msg}),z_0,z_1,e,u = z_0+z_1h+e\mod Q)$ in the random oracle storage.
%    \item for every signing query on $\mathsf{msg}$, $\mathcal S$ samples $\mathsf{salt}\overset{\$}{\leftarrow}\{0,1\}^{320}$, $\mathbf z=(\mathbf z_0,\mathbf z_1)\leftarrow D_{\mathbb Z^{2n},s}$ and $\mathbf e\leftarrow U(\mathbb Z_p^n)$, then output $(\mathsf{salt},\mathbf z_1)$ to $\mathcal A$ as the signature, and stores $((\mathsf{salt,msg}),\mathbf{z}_0,\mathbf z_1, \mathbf{e},\mathbf{A\cdot z+e}\mod Q)$ in the random oracle storage.
  \end{itemize}

Without loss of generality, assume that before outputting the signature forgery $(\mathsf{salt^*},z_1)$ for the message $\mathsf{msg^*}$, $\mathcal A$ queries $\mathsf H$ on $(\mathsf{salt}^*, \mathsf{msg^*})$. Then $\mathcal S$ computes $z'_0=\mathsf{H(salt^*,msg^*)}-z_1h\mod Q$ and looks up $((\mathsf{salt^*,msg^*}),z^*_0,z^*_1, e^*,u^*)$ in its local storage. Finally, $\mathcal S$ outputs $(z^*_0+e^*-z'_0,z^*_1-z_1)$ as a solution.
%and $(\mathbf z',\mathbf z_1)$ as a collision for $f_{\mathbf A}(\cdot)$.

By Theorem~\ref{thm:maintheorem}, the view of $\mathcal A$ in the real scheme is indistinguishable from the view provided by $\mathcal S$ except with negligible probability $Q_{sign}^2/2^{320}$, in which case repeated signature queries on the same message $\mathsf{msg}$ use the same $\mathsf{salt}$. It remains to prove that $z^*_1\neq z_1$. In fact, if $\mathsf{msg}^*$ has been queried to the signing oracle before, then the above inequality holds by the definition of a successful forgery; if $\mathsf{msg}^*$ has not been queried to the signing oracle, then $z_1$ is with high min-entropy for appropriate parameters, so $z^*_1\neq z_1$ with overwhelming probability.
\qed
\end{proof}

%
%The hash-and-sign signature scheme based on the approximate sampler in Theorem~\ref{thm:maintheorem} is specified by the following parameters.
%\begin{itemize}
%  \item modulus $Q=pq$;
%  \item hash function $\mathsf H:\{0,1\}^*\rightarrow\mathbb Z_Q^n$ modeled as a random oracle;
%  \item public key $\mathbf A=[\mathbf I_n\mid\hat{\mathbf A}]\in\mathbb Z_Q^{n\times m}$;
%  \item $l$ is the bit length of the $\mathsf{salt}$;
%  \item $r$ is the width for approximate gadget sampling: $r \geq q\bar{r}$ with $\bar{r} = \eta_{\epsilon}(\mathbb Z^n)$;
%  \item $s$ is the width for approximate preimage;
%  \item $\beta$ is the upper bound of $\|(\mathbf z_0+\mathbf e, \gamma \mathbf z_1)\|$ with $\gamma = \frac{\sqrt{s^2 + (p^2-1)/12}}{s}$
%    where $(\mathbf z_0,\mathbf z_1)\in\mathbb Z^{n}\times\mathbb Z^{m-n}$ is the approximate preimage and $\mathbf e$ is the approximate error.	
%\end{itemize}
%
%Now we are ready to construct the signature scheme.
%\begin{itemize}
%  \item $\mathsf{KeyGen}(1^n)$: Generate matrix $\mathbf A\in\mathbb Z_Q^{n\times m}$ together with its approximate gadget trapdoor $\mathbf T\in\mathbb Z^{m\times n}$ such that $\mathbf{A\cdot T}=p\mathbf I_n\mod Q$. Output $pk=\mathbf A$ and $sk=\mathbf T$.
%  \item $\mathsf{Sign}(\mathbf T, \mathsf{msg})$: Sample $\mathsf{salt}\overset{\$}{\leftarrow}\{0,1\}^{l}$ and compute $\mathbf u\leftarrow\mathsf{H(salt,msg)}$, then sample $\mathbf{z}\leftarrow\mathsf{ApproxPreSamp}\left(\mathbf A,\mathbf T,\mathbf u,r,s\right)$ where $\mathbf{z}=(\mathbf z_0,\mathbf z_1)\in\mathbb Z^{n}\times\mathbb Z^{m-n}$. Output $\mathsf{sig}=(\mathsf{salt,\mathbf z_1})$.
%  \item $\mathsf{Verify}(\mathbf A, \mathsf{msg},\mathsf{sig})$: Let $\mathbf z'=\mathsf{H(salt,msg)}-\hat{\mathbf{A}}\cdot\mathbf{z}_1\mod Q$. If $\|(\mathbf z', \gamma\mathbf z_1)\| \leq \beta$, output accept; otherwise, output reject.
%\end{itemize}
%
%\begin{theorem}
%  The scheme described above is strongly existentially unforgeable under a chosen-message attack in the random oracle model assuming the hardness of $\mathsf{SIS}_{n,m,q,2\beta}$.
%\end{theorem}
%
%\huiwen{The security is actually based on the hardness of finding the `scaled' short preimage. We need to define the asymmetric sis problem in $\ell_2$ norm?}






==> head/thmhead.tex <==
\theoremstyle{plain}            % following are "theorem" style
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{techlemma}[theorem]{Technical Lemma}

\newtheorem{maintheorem}{Main Theorem}

\theoremstyle{definition}       % following are def style
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{heuristic}[theorem]{Heuristic}
\newtheorem{construction}[theorem]{Construction}

\theoremstyle{remark}           % following are remark style
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{note}[theorem]{Note}

% equation numbering style
%\numberwithin{equation}{section}


==> scheme.tex <==
%!TEX root = main.tex
\section{Instantiation in the Ring Setting}
In this section, we provide a proof-of-concept implementation of our compact hash-and-sign signature scheme over the typical ring lattices. Recall the following parameters: $q=q_0\cdot q_1$, the lattice dimension $m=3n$, and $\sigma=q_1\cdot r$. Here we let $r=\sqrt{\log(2m(1+1/\epsilon))/\pi}$, where $\epsilon=1/\sqrt{Q_s\cdot\lambda}$, and $Q_s=2^{64}$ denotes the maximal number of signing queries, as in Falcon \cite{Falcon}.
$\Sigma=s_1^2\cdot\mathbf I_{2n}\oplus s_2^2\cdot\mathbf I_{n}$ is the Gaussian parameter for the approximate preimages, as in \cite{JHT22}.

Notice that the signature of a message essentially consists of two polynomials in $\mathbb Z_q[X]/(X^n+1)$, which coefficients are distributed around 0 with Gaussian parameters $s_1$ and $s_2$ respectively.
We fix $q=4095,q_0=819,q_1=5$ and use several groups of parameters with different $n,\tau$, and compare in Fig. 2 with the results in Falcon \cite{Falcon}, which has lattice dimension $2n$.

\vspace{-1em}

\begin{figure}\label{fig2}
	\centering
	\setlength{\tabcolsep}{1.5mm}
	%\linespread{1.5}
	\begin{tabular}{l|cccccccccc}
		\hline
		&$n$ & $q$ &$\tau$ & $s$      &$\beta$&Key Rec.&Forge&$\lambda$&$|pk|$& $|sig|$\\
		\hline
		Falcon&512 &12289& 4.05  & 415.4    & 5834  & 418    & 374 & 108     &897   &  808 \\
		Ours  &512 &4095 & 0.5   & (563,80) & 8968  & 298    & 298 & 79      &800   &  1384 \\
		\hline\hline
		Falcon&1024&12289& 2.87  & 422.1    & 8383  & 869    & 884 & 248     &1793  &  1576 \\
		Ours  &1024&4095 & 0.5   & (873,92) & 17650 & 706    & 652 & 173     &1568  &  2856 \\
		%\hline\hline
		%Ours  &2048&4095 & 0.25  &(880,102) & 27577 & 1352   &1451 & 358     &3104  &  5672\\
		\hline
	\end{tabular}
	\caption{A brief comparison of the parameters with Falcon \cite{Falcon}. Let $\tau$ be the standard deviation for secrets; $s$ the Gaussian parameter for the signatures; $\beta$ the norm threshold for signatures. `Key Rec.' and `Forge' refer to the estimated BKZ block size for recovering secret keys and forging signatures respectively. $\lambda$ denotes the security level in the quantum core-SVP model. $|pk|$ and $|sig|$ are in bytes. For $|pk|$ we use HNF and 32 bytes truly random string as seed to generate needed ring element. For $|sig|$, there are 40 bytes for the salts, and here we do not use the compression techniques to save storage.}
\end{figure} %\vspace{-1.5em}

%We use the most conservative evaluation model (quantum core-SVP) to estimate the concrete bit security, which sets the security level as 0.265$\kappa$, where $\kappa$ denotes the BKZ block size.

%We use `LWE security' to denote the pseudorandomness of the public key and `ISIS security' the hardness of solving the underlying ISIS problem.


\subsection{Security estimate}
We estimate concrete security by estimating how long it will take the BKZ algorithm to break the scheme. Specifically, the BKZ algorithm calls polynomial times a sieving subroutine to solve the exact SVP with dimension $\kappa$ (i.e., block size). We use the most conservative evaluation model (quantum core-SVP) to estimate the concrete security by setting the security level as 0.265$\kappa$ according to \cite{ADP+16}. As shown in Fig. \ref{fig2}, the concrete security of our instantiation relies on the pseudorandomness of the public key (`Key Rec.') and the hardness of solving the ISIS problem (`Forge').

`Key Rec.', i.e. LWE security, depends on the choices of $q, n$ and the standard deviation $\tau$ of the approximate trapdoor $\mathbf R$. We consider the primal attack and dual attack against the LWE problems.
\begin{itemize}
	\item For primal attack, the LWE samples $(\mathbf{A,b})\in\mathbb Z_q^{n\times m}\times\mathbb Z_q^{m}$ are converted to a unique-SVP instance for lattice
	$$
	\Lambda=\{\mathbf x\in\mathbb Z^{m+n+1}:(\mathbf{A}^t\mid\mathbf I\mid\mathbf b)\cdot\mathbf x=\mathbf 0\!\!\mod q\},
	$$
	then the BKZ algorithm is employed to recover the unique shortest vector $(\mathbf{s,e},1)$, which consists of the LWE secret and error vectors. As shown in \cite{ADP+16}, the attack is successful if and only if $\tau\sqrt{\kappa}\leq\delta^{2\kappa-d-1}\cdot q^{m/d}$, where $d=m+n+1$ and $\delta\approx\big(\frac{\kappa}{2\pi e}(\pi\kappa)^{1/\kappa}\big)^{1/2(\kappa-1)}$ is the root Hermite factor. \vspace{1em}
	\item For dual attack, the LWE samples $(\mathbf{A,b})\in\mathbb Z_q^{n\times m}\times\mathbb Z_q^{m}$ defines the lattice
	$$
	\Lambda=\{(\mathbf{x,y})\in\mathbb Z^m\times\mathbb Z^n:\mathbf A\cdot\mathbf x=\mathbf y\!\!\mod q\},
	$$
	and a short vector $\mathbf v\in\Lambda$ is helpful to solve the decisional LWE problem, i.e., distinguishing the distribution of $\mathbf{v}^t\cdot\mathbf b\!\!\mod q$ and the uniform distribution on $\mathbb Z_q$. According to \cite{ADP+16}, if the BKZ algorithm is capable of finding a short vector of length $\alpha=\delta^{d-1}q^{n/d}$, where $d=m+n$, then one can break the decisional LWE problem with advantage $\epsilon=4\exp(-2(\pi\alpha\tau/q)^2)$.
	
\end{itemize}


`Forge', i.e. the hardness of the ISIS problem, depends on the choices of $q, n$ and the norm bound $\beta$ of the preimage. Similarly, the security level estimation is based on how many operations BKZ would take to find a short vector with norm less than $\beta$ in lattice $\Lambda^{\bot}_q(\mathbf A)$. The BKZ algorithm is expected to find a vector of length $\delta^{d}\cdot\det(\Lambda^{\bot}_q(\mathbf A))^{1/d}$. Hence $\beta=\delta^{d}\cdot\det(\Lambda^{\bot}_q(\mathbf A))^{1/d}$ will determine $\delta$, which in turn can be used to figure out $\kappa$. Finally, the estimated security level will be $0.265\kappa$.

\subsection{Check the positivity of the covariance $\Sigma_{\mathbf p}$}
As mentioned early, when we use the rejection technique to set the Gaussian parameter $s$ for the preimages, we need an efficient algorithm to check whether $\Sigma_{\mathbf p}$ is positive definite or not. In this subsection, we present such an algorithm with optimal $\tilde O(n)$ time complexity.

For any $n\times n$ matrix $\mathbf{S}=\left[
\begin{array}{cc}
	\mathbf A & \mathbf B \\
	\mathbf C& \mathbf D \\
\end{array}
\right]$, the Schur complement of the square matrix $\mathbf A$ is defined to be $\mathbf{S/A=D-}\mathbf C\mathbf A^{-1}\mathbf B$. Particularly, if $\mathbf S$ is symmetric, then for any non-empty index sets $I\subset\{1,\ldots,n\}$, $\mathbf S$ is positive definite if and only if both $\mathbf S[I]$ and $\mathbf S/\mathbf S[I]$ are positive definite, where $\mathbf S[I]$ denotes the square matrix obtained by selecting the elements at positions $(i,j)\in I\times I$ from $\mathbf S$.

Recall that
\begin{equation*}
	\Sigma_{\mathbf{p}} = \left[
	\begin{array}{cc}
		s_1^2\cdot\mathbf I_{2n}-\sigma^2\cdot\mathbf{RR}^t & -\sigma^2\cdot\mathbf R \\
		-\sigma^2\cdot\mathbf R^t & (s_2^2-\sigma^2)\cdot\mathbf I_{nk_1}
	\end{array}
	\right],
\end{equation*}
then $\Sigma_{\mathbf{p}}>0$ if and only if $s_2>\sigma$ and $\Sigma_2=s_1^2\cdot\mathbf I_{2n}-\frac{s_2^2\sigma^2}{s_2^2-\sigma^2}\cdot\mathbf{RR}^t>0$. In the ring setting, $\Sigma_2$ is the matrix form of some rank 2 symmetric matrix over the typical ring $\mathcal Q=\mathbb Q[X]/(X^n+1)$ with $n$ being a power of 2. For ease of description, we treat the ring element $f\in\mathcal Q$ and the anti-circular matrix generated by $f$ as identical. Let $\Sigma_2=\left[
\begin{array}{cc}
	a & b \\
	b^t & d \\
\end{array}
\right]\in\mathcal Q^{2\times2}$, then $\Sigma_2>0$ if and only if $a-bd^{-1}b^t>0$ and $d>0$. The algorithm below describes how to check the positivity of symmetric $f\in\mathcal Q$. %\footnote{Here `symmetric' means that then anti-circular matrix generated by $f$ is symmetric.}

\begin{algorithm}[h]
	\setlength{\baselineskip}{13pt}
	\caption{\textsc{CheckF}}
	\begin{algorithmic}[1]
		\REQUIRE $f\in\mathcal Q$
		\ENSURE True or False
		\vspace{0.5em}
		\IF {dim($f$)=1}
		\IF{$f>0$}
		\RETURN True
		\ENDIF
		\RETURN False
		\ENDIF
		\STATE $f(X)=f_0(X^2)+X\cdot f_1(X^2)$
		\STATE $f'_0=f_0-f_1f_0^{-1}f_1^t$
		\RETURN \textsc{CheckF}($f'_0$) \&\& \textsc{CheckF}($f_0$)
	\end{algorithmic}
\end{algorithm}

Notice that \textsc{CheckF} is highly compatible with the perturbation sampling algorithm in \cite{GM18}, which requires recursive calls $\log n$ times, and each call needs to update the central vector and the covariance by computing $f_0f_1^{-1}$ and $f_0f_1^{-1}f_0$, respectively. Therefore, just as Falcon saves the binary tree during key generation, we could save the intermediate $f_0f_1^{-1}$ and $f_0f_1^{-1}f_0$ during each recursion by consuming a certain amount of space to reduce more than half of the computations in the perturbation sampling.

